Grafit: Learning fine-grained image representations with coarse labels

This paper tackles the problem of learning a finer representation than the one provided by training labels. This enables fine-grained category retrieval of images in a collection annotated with coarse labels only. Our network is learned with a nearest-neighbor classifier objective, and an instance loss inspired by self-supervised learning. By jointly leveraging the coarse labels and the underlying fine-grained latent space, it significantly improves the accuracy of category-level retrieval methods. Our strategy outperforms all competing methods for retrieving or classifying images at a finer granularity than that available at train time. It also improves the accuracy for transfer learning tasks to fine-grained datasets, thereby establishing the new state of the art on five public benchmarks, like iNaturalist-2018.

==> Figures_and_Tables/tables_inat/global_results.tex <==
\begin{tabular}{|ll|cccccccc|}
\toprule

&Test $\backslash$ Train & $\varnothing$ & King. & Phyl. & Class & Order & Fam. & Gen. & Spec. \\
\cmidrule{1-10} 
\multicolumn{10}{|c|}{iNaturalist-2018} \\
& \# classes: & 1 & 6 & 25 & 57 & 272 & 1118 & 4401 & 8142 \\
\cmidrule{1-10}

\multirow{7}{1em}{\rotatebox{90}{Baseline}}
& Kingdom   & 70.9   & 97.6      & 98.0     & 98.1     & 98.2      & 98.2     & 97.9       & 97.5  \\
& Phylum    & 48.8   & 88.0      & 96.3     & 96.4     & 96.6      & 96.7     & 96.2       & 95.2  \\
&Class     & 40.4   & 77.1      & 86.7     & 94.1     & 94.7      & 94.8     & 94.1       & 92.9  \\
&Order     & 17.1   & 43.6      & 55.0     & 61.0     & 85.6      & 86.6     & 85.5       & 82.6\\
&Family    & 5.6    &  23.0     & 32.8     & 36.7     & 62.0      & 80.7     & 79.7      & 76.1  \\
&Genus     & 0.9    & 10.0      & 17.3     & 20.1     & 41.7      & 63.0     & 72.5       & 68.3     \\
&Species   & 0.3    & 6.3       & 11.5     & 13.6     & 31.2      & 51.3     & 61.6       & 60.2  \\
\cmidrule{1-10}
\multirow{7}{1em}{\rotatebox{90}{SNCA+}}
&Kingdom   & 71.2   & 97.7      & 97.9     & 98.1     & 97.9      & 98.0     & 98.2       & 98.3  \\
&Phylum    & 48.0   & 68.7      & 96.1     & 96.4     & 96.4      & 96.5     & 96.7       & 96.7  \\
&Class     & 39.4   & 56.7      & 84.8     & 93.9     & 94.3      & 94.6     & 94.7       & 94.7  \\
&Order     & 16.2   & 23.3      & 47.4     & 59.0     & 85.4      & 86.2     & 86.7       & 86.7 \\
&Family    & 5.2   & 7.8      & 23.2       & 33.2        & 57.8      & 80.2     & 81.1       & 81.3  \\
&Genus     & 0.9   & 1.3      & 10.4       & 17.6       & 36.9      & 56.8     & 74.2       & 74.1    \\
&Species   & 0.3    & 0.5      & 6.3       & 11.9     & 26.2      & 42.4     & 58.9       & 64.6  \\
\cmidrule{1-10}
\multirow{7}{1em}{\rotatebox{90}{ClusterFit+}}
&Kingdom   & 70.9   & 94.7      & 95.0     & 95.3     & 95.6      & 96.2     & 96.3       & 96.1  \\
&Phylum    & 48.8   & 87.4      & 90.3     & 90.7     & 91.1      & 92.6     & 92.6       & 92.2  \\
&Class     & 40.4   & 80.2      & 83.8     & 85.7     & 86.7      & 88.8     & 88.8       & 88.2  \\
&Order     & 17.1   & 54.5      & 59.0     & 61.4     & 70.8      & 73.9     & 74.3       & 72.3  \\
&Family    & 5.6   & 38.3      & 42.1     & 44.4     & 54.3      & 63.0    & 64.2       & 61.9  \\
&Genus     & 0.9   & 26.7      & 29.5     & 31.5     & 40.1      & 49.4     & 53.9       & 51.7  \\
&Species  & 0.3   & 21.8      & 23.7     & 25.2     & 32.7      & 40.3     & 44.7       & 43.4  \\

\cmidrule{1-10}
\multirow{7}{1em}{\rotatebox{90}{\ours FC}}
&Kingdom   & 91.1   & 97.8      & 98.1     & 98.4     & 98.3      & 98.4     & 98.5       & 98.4       \\
&Phylum    & 81.7   & 93.0      & 96.4     & 96.9     & 97.0      & 96.9     & 97.1       & 96.8       \\
&Class     & 71.9   & 86.0      & 90.7     & 94.8     & 95.0      & 95.1     & 95.3       & 95.0       \\
&Order     & 41.8   & 58.5      & 66.8     & 72.2     & 86.8      & 87.1     & 87.3       & 87.2       \\
&Family    & 22.4   & 38.8      & 48.4     & 54.4     & 70.4      & 81.1     & 81.6       & 81.7       \\
&Genus     & 11.4   & 24.6      & 33.1     & 38.6     & 53.0      & 63.9     & 73.8       & 74.2       \\
&Species   & 8.13   & 18.8      & 25.6     & 29.9     & 41.5      & 50.9     & 60.9       & 65.9       \\

\cmidrule{1-10}
\multirow{7}{1em}{\rotatebox{90}{\ours}}
&Kingdom   & 95.5   & 98.1      & 98.2     & 98.2     & 98.2      & 98.2     & 98.4       & 98.3       \\
&Phylum    & 90.0   & 94.1      & 96.6     & 96.7     & 96.8      & 96.7     & 96.9       & 96.7       \\
&Class     & 82.2   & 87.5      & 90.9     & 94.5     & 94.9      & 94.9     & 95.0       & 95.0       \\
&Order     & 54.0   & 61.7      & 66.9     & 72.7     & 87.1      & 87.5     & 87.6       & 87.3       \\
&Family    & 33.7   & 42.1      & 48.7     & 55.1     & 70.9      & 81.8     & 82.4       & 82.1       \\
&Genus     & 20.5   & 27.0      & 33.5     & 39.5     & 54.2      & 64.6     & 75.6       & 75.5       \\
&Species   & 15.9   & 20.4      & 25.5     & 30.8     & 42.7      & 51.2     & 61.9       & 67.7       \\

\midrule

\multicolumn{10}{|c|}{iNaturalist-2019} \\
& \# classes: & 1 & 3 & 4 & 9 & 34 & 57 & 72 & 1010 \\
% &Test $\backslash$ Train & $\varnothing$ & King. & Phyl. & Class & Order & Fam. & Gen. & Spec. \\
\cmidrule{1-10}

\multirow{7}{1em}{\rotatebox{90}{Baseline}}
&Kingdom   & 77.0   & 98.9      & 98.9     & 99.0     & 99.3      & 99.4     & 99.3       & 98.9       \\
&Phylum    & 73.8   & 97.1      & 98.7     & 98.9     & 99.2      & 99.2     & 99.2       & 98.7       \\
&Class     & 63.3   & 87.6      & 90.3     & 98.0     & 98.5      & 98.6     & 98.6       & 98.0      \\
&Order     & 17.9   & 49.6      & 56.4     & 70.8     & 95.6      & 95.5     & 96.0       & 95.2      \\
&Family    & 12.4   & 42.1      & 50.4     & 65.0     & 89.4      & 94.8     & 95.1       & 94.4     \\
&Genus     & 9.6   & 39.2       & 46.5     & 62.1     & 86.1      & 91.5     & 94.8       & 93.9     \\
&Species   & 1.5   & 9.8        & 13.5     & 20.6     & 34.5      & 39.9     & 42.4       & 75.0     \\
\cmidrule{1-10}
\multirow{7}{1em}{\rotatebox{90}{SNCA+}}
&Kingdom   & 76.9   & 98.6      & 98.9     & 99.2     & 99.2      & 99.3     & 99.1       & 99.0  \\
&Phylum    & 73.3   & 87.1      & 98.8     & 99.1     & 99.1      & 99.1     & 98.9       & 99.0  \\
&Class     & 62.3   & 74.9      & 84.1     & 98.2     & 98.6      & 98.3     & 98.1       & 97.8  \\
&Order     & 17.6   & 19.7      & 30.2     & 55.4     & 95.3      & 95.2     & 95.2       & 94.2 \\
&Family    & 12.2   & 12.7      & 20.7     & 45.5     & 88.2      & 94.5     & 94.6       & 93.5  \\
&Genus     & 9.3    & 9.2      & 17.1      & 41.6     & 85.0      & 91.2     & 94.0        & 93.1    \\
&Species   & 1.3    & 1.0      & 1.8       & 10.4     & 36.0      & 40.8     & 42.3       & 74.7  \\
\cmidrule{1-10}
\multirow{7}{1em}{\rotatebox{90}{ClusterFit+}}
&Kingdom   & 77.0   & 96.4      & 96.1     & 95.8     & 95.7      & 95.7     & 95.4       & 97.0  \\
&Phylum    & 73.8   & 94.2      & 95.0     & 94.6     & 94.3      & 94.4     & 93.8       & 95.5  \\
&Class     & 63.3   & 88.7      & 90.1     & 91.3     & 90.1      & 90.9     & 90.6       & 93.5  \\
&Order     & 17.9   & 65.5      & 67.9     & 70.9     & 76.8      & 79.0     & 78.1       & 83.2  \\
&Family    & 12.4   & 59.5      & 62.0     & 65.4     & 71.7      & 75.6     & 75.3       & 80.4  \\
&Genus     & 9.6   & 56.9      & 59.3     & 62.7     & 68.7      & 72.6     & 73.9       & 78.6  \\
&Species  & 1.5   & 24.5      & 25.6     & 27.3     & 31.1      & 33.6     & 33.9       & 49.6  \\
\cmidrule{1-10}
\multirow{7}{1em}{\rotatebox{90}{\ours FC}}
&Kingdom   & 93.1   & 98.9      & 99.0     & 99.2     & 99.2      & 99.4     & 99.4       & 99.2       \\
&Phylum    & 90.9   & 98.2      & 98.9     & 99.1     & 99.1      & 99.3     & 99.2       & 99.0       \\
&Class     & 82.6   & 94.9      & 96.4     & 98.2     & 98.3      & 98.7     & 98.7       & 98.3       \\
&Order     & 52.5   & 80.0      & 83.5     & 89.5     & 95.8      & 96.0     & 95.9       & 95.3       \\
&Family    & 45.3   & 74.6      & 78.9     & 86.0     & 93.4      & 95.2     & 95.4       & 94.7       \\
&Genus     & 41.7   & 71.7      & 76.3     & 84.0     & 91.7      & 93.4     & 95.0       & 94.3       \\
&Species   & 12.0   & 29.5      & 32.6     & 40.4     & 51.8      & 53.2     & 53.9       & 75.9       \\
\cmidrule{1-10}
\multirow{7}{1em}{\rotatebox{90}{\ours}}
&Kingdom   & 96.9   & 99.2      & 99.1     & 99.2     & 99.2      & 99.0     & 99.0       & 99.0\\
&Phylum    & 96.4   & 98.8      & 98.9     & 99.0     & 99.0      & 98.9     & 98.9       & 98.7\\
&Class     & 93.0   & 97.0      & 97.1     & 98.2     & 98.4      & 98.3     & 98.1       & 97.8\\
&Order     & 81.3   & 89.0      & 89.3     & 91.2     & 95.9      & 95.3     & 95.3       & 94.5\\
&Family    & 76.5   & 85.2      & 85.2     & 87.8     & 93.1      & 94.5     & 94.5       & 93.8\\
&Genus     & 73.8   & 82.7      & 83.1     & 85.8     & 91.3      & 92.6     & 94.2       & 93.4\\
&Species   & 31.0   & 41.6      & 41.4     & 46.0     & 51.8      & 53.5     & 55.3      & 75.3\\


\bottomrule
\end{tabular}

==> Figures_and_Tables/tables_inat/our_method_knn.tex <==
\begin{tabular}{c|l|cccccccc}
\toprule
\toprule
\multicolumn{9}{c}{\ours}\\

\multirow{8}{2em}{\rotatebox{90}{iNaturalist-2018}}  &Test / Train & $\emptyset$ & Kingdom & Phylum & class & Order & Family & Genus & Species \\
\cmidrule{2-10}

&Kingdom   & 95.5   & 98.1      & 98.2     & 98.2     & 98.2      & 98.2     & 98.4       & 98.3       \\
&Phylum    & 90.0   & 94.1      & 96.6     & 96.7     & 96.8      & 96.7     & 96.9       & 96.7       \\
&class     & 82.2   & 87.5      & 90.9     & 94.5     & 94.9      & 94.9     & 95.0       & 95.0       \\
&Order     & 54.0   & 61.7      & 66.9     & 72.7     & 87.1      & 87.5     & 87.6       & 87.3       \\
&Family    & 33.7   & 42.1      & 48.7     & 55.1     & 70.9      & 81.8     & 82.4       & 82.1       \\
&Genus     & 20.5   & 27.0      & 33.5     & 39.5     & 54.2      & 64.6     & 75.6       & 75.5       \\
&Species   & 15.9   & 20.4      & 25.5     & 30.8     & 42.7      & 51.2     & 61.9       & 67.7       \\
\midrule
\multirow{8}{2em}{\rotatebox{90}{iNaturalist-2019}} &Test / Train & $\emptyset$ & Kingdom & Phylum & class & Order & Family & Genus & Species \\
\cmidrule{2-10}
 
&Kingdom   & 96.9   & 99.2      & 99.1     & 99.2     & 99.2      & 99.0     & 99.0       & 99.0\\
&Phylum    & 96.4   & 98.8      & 98.9     & 99.0     & 99.0      & 98.9     & 98.9       & 98.7\\
&class     & 93.0   & 97.0      & 97.1     & 98.2     & 98.4      & 98.3     & 98.1       & 97.8\\
&Order     & 81.3   & 89.0      & 89.3     & 91.2     & 95.9      & 95.3     & 95.3       & 94.5\\
&Family    & 76.5   & 85.2      & 85.2     & 87.8     & 93.1      & 94.5     & 94.5       & 93.8\\
&Genus     & 73.8   & 82.7      & 83.1     & 85.8     & 91.3      & 92.6     & 94.2       & 93.4\\
&Species   & 31.0   & 41.6      & 41.4     & 46.0     & 51.8      & 53.5     & 55.3      & 75.3\\
\bottomrule
\end{tabular}

==> ablation.tex <==
\section{Ablation studies}
\label{sec:ablation}

\paragraph{Losses, architectural choice and conditioning.} 
Table~\ref{tab:Ablation_baselines_coarse_to_fine} presents a study on CIFAR-100 and ImageNet-1k, where we ablate several components of our method.
A large improvement stems from the instance loss when it supplements the supervised kNN loss. It is key for discriminating at a finer grain. 
The category-level retrieval significantly benefit from our approach, rising from 22.7 to 44.4 in the best case. 

\input{Figures_and_Tables/tab_Ablation_baselines_coarse_to_fine_v2}

\paragraph{Sanity check: training with coarse vs fine labels. } 
% 
% 
Table~\ref{tab:coarse_to_fine_fine_to_fine} compares the performance gap of several methods when training with coarse labels vs of fine labels. \ours significantly reduces the loss of accuracy resulting from the reduced label granularity. This concurs with our prior observations in Section~\ref{sec:sub_category_disc} on iNaturalist-2018. See Appendix~\ref{app:experiment} for additional results on Imagenet. 
% 
Overall, in this setting \ours provides some slight yet systematic improvement over the baseline. 
With a ResNet-50 architecture  at image resolution $224 \times 224$ pixels, \ours  reaches \textbf{79.6\%} top-1 accuracy with a \knn classifier on ImageNet. 





\input{Figures_and_Tables/tab:coarse_to_fine_fine_to_fine}



